Sequence Complementor: Complementing Transformers For Time Series Forecasting with Learnable Sequences

Since its introduction, the transformer has shifted the development trajectory away from traditional models (e.g., RNN, MLP) in time series forecasting, which is attributed to its ability to capture global dependencies within temporal tokens. Follow-up studies have largely involved altering the tokenization and self-attention modules to better adapt Transformers for addressing special challenges like non-stationarity, channel-wise dependency, and variable correlation in time series. However, we found that the expressive capability of sequence representation is a key factor influencing Transformer performance in time forecasting after investigating several representative methods, where there is an almost linear relationship between sequence representation entropy and mean square error, with more diverse representations performing better. In this paper, we propose a novel attention mechanism with Sequence Complementors and prove feasible from an information theory perspective, where these learnable sequences are able to provide complementary information beyond current input to feed attention. We further enhance the Sequence Complementors via a diversification loss that is theoretically covered. The empirical evaluation of both long-term and short-term forecasting has confirmed its superiority over the recent state-of-the-art methods.

==> table-short-backup.tex <==

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \centering
% \caption{}
% \label{tab:short-term}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clccccccccccccccc}
% \multicolumn{2}{c}{\textbf{Models}} & \textbf{Ours} & \textbf{\begin{tabular}[c]{@{}c@{}}CARD \\  ICLR'24\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PatchTST\\  ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Crossformer \\    ICLR'XX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FEDformer \\    XXXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RMLP \\  XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rlinear\\ XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MTS-mixer \\ XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LightTS \\  XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DLinear \\  AAAI'xxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TimesNet\\  ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SCINet \\  xxxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FEDformer\\  XXXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Non-Stat.\\  xxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Autoformer\\  XXXX\end{tabular}} \\
%  & SMAPE & {\color[HTML]{FF0000} 13.185} & 13.302 & {\color[HTML]{0000FF} 13.258} & 13.392 & 13.728 & 13.418 & 13.994 & 13.548 & 14.247 & 16.965 & 13.387 & 13.717 & 13.728 & 13.717 & 13.974 \\
%  & MASE & {\color[HTML]{FF0000} 2.955} & 3.016 & {\color[HTML]{0000FF} 2.985} & 3.001 & 3.048 & 3.006 & 3.015 & 3.091 & 3.109 & 4.283 & 2.996 & 3.076 & 3.048 & 3.078 & 3.134 \\
% \multirow{-3}{*}{Year} & OWA & {\color[HTML]{FF0000} 0.775} & 0.786 & {\color[HTML]{0000FF} 0.781} & 0.787 & 0.803 & 0.789 & 0.807 & 0.803 & 0.827 & 1.058 & 0.786 & 0.807 & 0.803 & 0.807 & 0.822 \\
%  & SMAPE & {\color[HTML]{FF0000} 9.989} & {\color[HTML]{0000FF} 10.031} & 10.179 & 16.317 & 10.792 & 10.382 & 10.702 & 10.128 & 11.364 & 12.145 & 10.1 & 10.845 & 10.792 & 10.958 & 11.338 \\
%  & MASE & {\color[HTML]{0000FF} 1.17} & 1.176 & {\color[HTML]{FF0000} 0.803} & 2.197 & 1.283 & 1.234 & 1.299 & 1.196 & 1.328 & 1.52 & 1.182 & 1.295 & 1.283 & 1.325 & 1.365 \\
% \multirow{-3}{*}{Quarterly} & OWA & {\color[HTML]{0000FF} 0.88} & 0.884 & {\color[HTML]{FF0000} 0.803} & 1.542 & 0.958 & 0.921 & 0.959 & 0.896 & 1 & 1.106 & 0.89 & 0.965 & 0.958 & 0.981 & 1.012 \\
%  & SMAPE & {\color[HTML]{FF0000} 12.453} & 12.67 & {\color[HTML]{0000FF} 12.641} & 12.924 & 14.26 & 12.998 & 13.363 & 12.717 & 14.014 & 13.514 & 12.67 & 13.208 & 14.26 & 13.917 & 13.958 \\
%  & MASE & {\color[HTML]{FF0000} 0.913} & 0.933 & {\color[HTML]{0000FF} 0.93} & 0.966 & 1.102 & 0.976 & 1.014 & 0.931 & 1.053 & 1.037 & 0.933 & 0.999 & 1.102 & 1.097 & 1.103 \\
% \multirow{-3}{*}{Monthly} & OWA & {\color[HTML]{FF0000} 0.861} & 0.878 & {\color[HTML]{0000FF} 0.876} & 0.902 & 1.012 & 0.909 & 0.94 & 0.879 & 0.981 & 0.956 & 0.878 & 0.928 & 1.012 & 0.998 & 1.002 \\
%  & SMAPE & {\color[HTML]{FF0000} 4.565} & 5.33 & 4.946 & 5.439 & 4.954 & 5.098 & 5.437 & {\color[HTML]{0000FF} 4.817} & 15.88 & 6.709 & 4.891 & 5.432 & 4.954 & 6.302 & 5.458 \\
%  & MASE & {\color[HTML]{0000FF} 3.144} & 3.261 & {\color[HTML]{FF0000} 2.985} & 3.69 & 3.264 & 3.364 & 3.706 & 3.255 & 11.434 & 4.953 & 3.302 & 3.583 & 3.264 & 4.064 & 3.865 \\
% \multirow{-3}{*}{Others} & OWA & {\color[HTML]{FF0000} 0.976} & 1.075 & 1.044 & 1.16 & 1.036 & 1.067 & 1.157 & {\color[HTML]{0000FF} 1.02} & 3.474 & 1.487 & 1.035 & 1.136 & 1.036 & 1.304 & 1.187 \\
%  & SMAPE & {\color[HTML]{FF0000} 11.636} & 11.815 & {\color[HTML]{0000FF} 11.807} & 13.474 & 12.84 & 12.473 & 12.473 & 11.892 & 13.252 & 13.639 & 11.829 & 12.369 & 12.84 & 12.78 & 12.909 \\
%  & MASE & {\color[HTML]{FF0000} 1.556} & 1.587 & 1.59 & 1.866 & 1.701 & 1.677 & 1.677 & 1.608 & 2.111 & 2.095 & {\color[HTML]{0000FF} 1.585} & 1.677 & 1.701 & 1.756 & 1.771 \\
% \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Weighted\\      Average\end{tabular}} & OWA & {\color[HTML]{FF0000} 0.836} & {\color[HTML]{0000FF} 0.85} & 0.851 & 0.985 & 0.918 & 0.898 & 0.898 & 0.859 & 1.051 & 0.851 & 0.851 & 0.894 & 0.918 & 0.93 & 0.939
% \end{tabular}%
% }
% \end{table}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\caption{}
\label{tab:LONG}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc} \toprule
\multicolumn{2}{c}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Ours}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}iTransformer\\      ICLR'24\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Rlinear\\      XXXX\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}PatchTST\\      ICLR'23\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Crossformer\\      xxxx\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}TimesNet\\      ICLR'23\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Dlinear\\      AAAI'XXX\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}SCINet\\      xxxxx\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}FEDformer\\      XXXXX\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Stationary\\      xxxxxx\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Autoformer\\      XXXXX\end{tabular}}} \\
\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \midrule
 & 96 &\textbf{ 0.321} &\textbf{ 0.359} & 0.334 & 0.368 & 0.355 & 0.376 & \underline{0.329} & \underline{0.367} & 0.404 & 0.426 & 0.338 & 0.375 & 0.345 & 0.372 & 0.418 & 0.438 & 0.379 & 0.419 & 0.386 & 0.398 & 0.505 & 0.475 \\
 & 192 &\textbf{ 0.362} &\underline{ 0.386} & 0.377 & 0.391 & 0.391 & 0.392 &\underline{ 0.367} &\textbf{ 0.385} & 0.450 & 0.451 & 0.374 & 0.387 & 0.380 & 0.389 & 0.439 & 0.450 & 0.426 & 0.441 & 0.459 & 0.444 & 0.553 & 0.496 \\
 & 336 &\textbf{ 0.393} &\textbf{ 0.406} & 0.426 & 0.420 & 0.424 & 0.415 &\underline{ 0.399} &\underline{ 0.410} & 0.532 & 0.515 & 0.410 & 0.411 & 0.413 & 0.413 & 0.490 & 0.485 & 0.445 & 0.459 & 0.495 & 0.464 & 0.621 & 0.537 \\
 & 720 &\textbf{ 0.450} &\underline{ 0.442} & 0.491 & 0.459 & 0.487 & 0.450 &\underline{ 0.454} &\textbf{ 0.439} & 0.666 & 0.589 & 0.478 & 0.450 & 0.474 & 0.453 & 0.595 & 0.550 & 0.543 & 0.490 & 0.585 & 0.516 & 0.671 & 0.561 \\ 
\multirow{-5}{*}{ETTm1} & avg &\textbf{ 0.381} &\textbf{ 0.398} & 0.407 & 0.410 & 0.414 & 0.408 &\underline{ 0.387} &\underline{ 0.400} & 0.513 & 0.495 & 0.400 & 0.406 & 0.403 & 0.407 & 0.486 & 0.481 & 0.448 & 0.452 & 0.481 & 0.456 & 0.588 & 0.517 \\  \midrule
 & 96 &\textbf{ 0.115} &\textbf{ 0.227} & 0.180 & 0.264 & 0.182 & 0.265 &\underline{ 0.175} &\underline{ 0.259} & 0.287 & 0.366 & 0.187 & 0.267 & 0.193 & 0.292 & 0.286 & 0.377 & 0.203 & 0.287 & 0.192 & 0.274 & 0.255 & 0.339 \\
 & 192 &\textbf{ 0.145} &\textbf{ 0.259} & 0.250 & 0.309 & 0.246 & 0.304 &\underline{ 0.241} &\underline{ 0.302} & 0.414 & 0.492 & 0.249 & 0.309 & 0.284 & 0.362 & 0.399 & 0.445 & 0.269 & 0.328 & 0.280 & 0.339 & 0.281 & 0.340 \\
 & 336 &\textbf{ 0.180} &\textbf{ 0.288} & 0.311 & 0.348 & 0.307 &\underline{ 0.342} &\underline{ 0.305} & 0.343 & 0.597 & 0.542 & 0.321 & 0.351 & 0.369 & 0.427 & 0.637 & 0.591 & 0.325 & 0.366 & 0.334 & 0.361 & 0.339 & 0.372 \\
 & 720 &\textbf{ 0.237} &\textbf{ 0.330} & 0.412 & 0.407 & 0.407 &\underline{ 0.398} &\underline{ 0.402} & 0.400 & 1.730 & 1.042 & 0.408 & 0.403 & 0.554 & 0.522 & 0.960 & 0.735 & 0.421 & 0.415 & 0.417 & 0.413 & 0.433 & 0.432 \\  
\multirow{-5}{*}{ETTm2} & avg &\textbf{ 0.169} &\textbf{ 0.276} & 0.288 & 0.332 & 0.286 & 0.327 &\underline{ 0.281} &\underline{ 0.326} & 0.757 & 0.611 & 0.291 & 0.333 & 0.350 & 0.401 & 0.571 & 0.537 & 0.305 & 0.349 & 0.306 & 0.347 & 0.327 & 0.371 \\  \midrule
 & 96 &\textbf{ 0.375} &\textbf{ 0.394} & 0.386 & 0.405 & 0.386 &\underline{ 0.395} & 0.414 & 0.419 & 0.423 & 0.448 & 0.384 & 0.402 & 0.386 & 0.400 & 0.654 & 0.599 &\underline{ 0.376} & 0.429 & 0.513 & 0.491 & 0.449 & 0.459 \\
 & 192 &\underline{ 0.423} &\underline{ 0.425} & 0.441 & 0.436 & 0.437 &\textbf{ 0.424} & 0.460 & 0.445 & 0.471 & 0.474 & 0.436 & 0.429 & 0.437 & 0.432 & 0.719 & 0.631 &\textbf{ 0.420} & 0.448 & 0.534 & 0.504 & 0.500 & 0.482 \\
 & 336 &\textbf{ 0.457} &\underline{ 0.448} & 0.487 & 0.458 & 0.479 &\textbf{ 0.446} & 0.501 & 0.466 & 0.570 & 0.546 & 0.491 & 0.469 & 0.481 & 0.459 & 0.778 & 0.659 &\underline{ 0.459} & 0.465 & 0.588 & 0.535 & 0.521 & 0.496 \\
 & 720 &\textbf{ 0.462} &\underline{ 0.472} & 0.503 & 0.491 &\underline{ 0.481} &\textbf{ 0.470} & 0.500 & 0.488 & 0.653 & 0.621 & 0.521 & 0.500 & 0.519 & 0.516 & 0.836 & 0.699 & 0.506 & 0.507 & 0.643 & 0.616 & 0.514 & 0.512 \\ 
\multirow{-5}{*}{ETTh1} & avg &\textbf{ 0.429} &\underline{ 0.435} & 0.454 & 0.448 & 0.446 &\textbf{ 0.434} & 0.469 & 0.455 & 0.529 & 0.522 & 0.458 & 0.450 & 0.456 & 0.452 & 0.747 & 0.647 &\underline{ 0.440} & 0.462 & 0.570 & 0.537 & 0.496 & 0.487 \\  \midrule
 & 96 & 0.283 &\underline{ 0.337} & 0.297 & 0.349 & 0.288 & 0.338 & 0.302 & 0.348 & 0.745 & 0.584 & 0.340 & 0.374 & 0.333 & 0.387 & 0.707 & 0.621 &\textbf{ 0.036} &\textbf{ 0.040} &\underline{ 0.048} & 0.458 & 0.346 & 0.388 \\
 & 192 &\textbf{ 0.362} &\textbf{ 0.388} & 0.380 & 0.400 &\underline{ 0.374} &\underline{ 0.390} & 0.388 & 0.400 & 0.877 & 0.656 & 0.402 & 0.414 & 0.477 & 0.476 & 0.860 & 0.689 & 0.429 & 0.439 & 0.512 & 0.493 & 0.456 & 0.452 \\
 & 336 &\textbf{ 0.408} &\textbf{ 0.425} & 0.428 & 0.432 &\underline{ 0.415} &\underline{ 0.426} & 0.426 & 0.433 & 1.043 & 0.731 & 0.452 & 0.452 & 0.594 & 0.541 & 1.000 & 0.744 & 0.496 & 0.487 & 0.552 & 0.551 & 0.482 & 0.486 \\
 & 720 &\textbf{ 0.419} &\underline{ 0.441} & 0.427 & 0.445 &\underline{ 0.420} &\textbf{ 0.440} & 0.431 & 0.446 & 1.104 & 0.763 & 0.462 & 0.468 & 0.831 & 0.657 & 1.249 & 0.838 & 0.463 & 0.474 & 0.562 & 0.560 & 0.515 & 0.511 \\  
\multirow{-5}{*}{ETTh2} & avg &\underline{ 0.368} &\underline{ 0.398} & 0.383 & 0.407 & 0.374 & 0.399 & 0.387 & 0.407 & 0.942 & 0.684 & 0.414 & 0.427 & 0.559 & 0.515 & 0.954 & 0.723 &\textbf{ 0.356} &\textbf{ 0.360} & 0.418 & 0.516 & 0.450 & 0.459 \\  \midrule
 & 96 &\underline{ 0.156} &\underline{ 0.252} &\textbf{ 0.148} &\textbf{ 0.240} & 0.201 & 0.281 & 0.181 & 0.270 & 0.219 & 0.314 & 0.168 & 0.272 & 0.197 & 0.282 & 0.247 & 0.345 & 0.193 & 0.308 & 0.169 & 0.273 & 0.201 & 0.317 \\
 & 192 &\underline{ 0.175} &\underline{ 0.269} &\textbf{ 0.162} &\textbf{ 0.253} & 0.201 & 0.283 & 0.188 & 0.274 & 0.231 & 0.322 & 0.184 & 0.289 & 0.196 & 0.285 & 0.257 & 0.355 & 0.201 & 0.315 & 0.182 & 0.286 & 0.222 & 0.334 \\
 & 336 &\underline{ 0.190} &\underline{ 0.284} &\textbf{ 0.178} &\textbf{ 0.269} & 0.215 & 0.298 & 0.204 & 0.293 & 0.246 & 0.337 & 0.198 & 0.300 & 0.209 & 0.301 & 0.269 & 0.369 & 0.214 & 0.329 & 0.200 & 0.304 & 0.231 & 0.338 \\
 & 720 & 0.246 & 0.324 & 0.225 &\textbf{ 0.317} & 0.257 & 0.331 & 0.246 & 0.324 & 0.280 & 0.363 &\textbf{ 0.220} &\underline{ 0.320} & 0.245 & 0.333 & 0.299 & 0.390 & 0.246 & 0.355 &\underline{ 0.222} & 0.321 & 0.254 & 0.361 \\ 
\multirow{-5}{*}{ECL} & avg &\underline{ 0.192} &\underline{ 0.282} &\textbf{ 0.178} &\textbf{ 0.270} & 0.219 & 0.298 & 0.205 & 0.290 & 0.244  & 0.334 & 0.193 & 0.295 & 0.212 & 0.300 & 0.268 & 0.365 & 0.214 & 0.327 & 0.193 & 0.296 & 0.227 & 0.338 \\  \midrule
 & 96 &\textbf{ 0.082} &\textbf{ 0.200} &\underline{ 0.086} & 0.206 & 0.093 & 0.217 & 0.088 &\underline{ 0.205} & 0.256 & 0.367 & 0.107 & 0.234 & 0.088 & 0.218 & 0.267 & 0.396 & 0.148 & 0.278 & 0.111 & 0.237 & 0.197 & 0.323 \\
 & 192 &\textbf{ 0.175} &\textbf{ 0.297} & 0.177 &\underline{ 0.299} & 0.184 & 0.307 &\underline{ 0.176} & 0.299 & 0.470 & 0.509 & 0.226 & 0.344 & 0.176 & 0.315 & 0.351 & 0.459 & 0.271 & 0.315 & 0.219 & 0.335 & 0.300 & 0.369 \\
 & 336 & 0.325 &\underline{ 0.413} & 0.331 & 0.419 & 0.351 & 0.432 &\textbf{ 0.301} &\textbf{ 0.397} & 1.268 & 0.883 & 0.367 & 0.448 &\underline{ 0.313} & 0.427 & 1.324 & 0.853 & 0.460 & 0.427 & 0.421 & 0.476 & 0.509 & 0.524 \\
 & 720 &\underline{ 0.840} &\textbf{ 0.690} & 0.847 &\underline{ 0.691} & 0.886 & 0.714 & 0.901 & 0.714 & 1.767 & 1.068 & 0.964 & 0.746 &\textbf{ 0.839} & 0.695 & 1.058 & 0.797 & 1.195 & 0.695 & 1.092 & 0.769 & 1.447 & 0.941 \\ 
\multirow{-5}{*}{Exchange} & avg &\underline{ 0.356} &\textbf{ 0.400} & 0.360 &\underline{ 0.404} & 0.379 & 0.418 & 0.367 & 0.404 & 0.940 & 0.707 & 0.416 & 0.443 &\textbf{ 0.354} & 0.414 & 0.750 & 0.626 & 0.519 & 0.429 & 0.461 & 0.454 & 0.613 & 0.539 \\  \midrule
 & 96 &\underline{ 0.455} & 0.291 &\textbf{ 0.395} &\textbf{ 0.268} & 0.649 & 0.389 & 0.462 & 0.295 & 0.522 &\underline{ 0.290} & 0.593 & 0.321 & 0.650 & 0.396 & 0.788 & 0.499 & 0.587 & 0.366 & 0.612 & 0.338 & 0.613 & 0.388 \\
 & 192 &\underline{ 0.460} &\underline{ 0.291} &\textbf{ 0.417} &\textbf{ 0.276} & 0.601 & 0.366 & 0.466 & 0.296 & 0.530 & 0.293 & 0.617 & 0.336 & 0.598 & 0.370 & 0.789 & 0.505 & 0.604 & 0.373 & 0.613 & 0.340 & 0.616 & 0.382 \\
 & 336 &\underline{ 0.473} &\underline{ 0.302} &\textbf{ 0.433} &\textbf{ 0.283} & 0.609 & 0.369 & 0.482 & 0.304 & 0.558 & 0.305 & 0.629 & 0.336 & 0.605 & 0.373 & 0.797 & 0.508 & 0.621 & 0.383 & 0.618 & 0.328 & 0.622 & 0.337 \\
 & 720 &\underline{ 0.500} &\underline{ 0.321} &\textbf{ 0.467} &\textbf{ 0.302} & 0.647 & 0.387 & 0.514 & 0.322 & 0.589 & 0.328 & 0.640 & 0.350 & 0.645 & 0.394 & 0.841 & 0.523 & 0.626 & 0.382 & 0.653 & 0.355 & 0.660 & 0.408 \\  
\multirow{-5}{*}{Traffic} & avg &\underline{ 0.472} &\underline{ 0.301} &\textbf{ 0.428} &\textbf{ 0.282} & 0.627 & 0.378 & 0.481 & 0.304 & 0.550 & 0.304 & 0.620 & 0.336 & 0.625 & 0.383 & 0.804 & 0.509 & 0.610 & 0.376 & 0.624 & 0.340 & 0.628 & 0.379 \\  \midrule
 & 96 &\underline{ 0.159} &\textbf{ 0.206} & 0.174 &\underline{ 0.214} & 0.192 & 0.232 & 0.177 & 0.218 &\textbf{ 0.158} & 0.230 & 0.172 & 0.220 & 0.196 & 0.255 & 0.221 & 0.306 & 0.217 & 0.296 & 0.173 & 0.223 & 0.266 & 0.336 \\
 & 192 &\textbf{ 0.205} &\textbf{ 0.249} & 0.221 &\underline{ 0.254} & 0.240 & 0.271 & 0.225 & 0.259 &\underline{ 0.206} & 0.277 & 0.219 & 0.261 & 0.237 & 0.296 & 0.261 & 0.340 & 0.276 & 0.336 & 0.245 & 0.285 & 0.307 & 0.367 \\
 & 336 &\textbf{ 0.263} &\textbf{ 0.291} & 0.278 &\underline{ 0.296} & 0.292 & 0.307 & 0.278 & 0.297 &\underline{ 0.272} & 0.335 & 0.280 & 0.306 & 0.283 & 0.335 & 0.309 & 0.378 & 0.339 & 0.380 & 0.321 & 0.338 & 0.359 & 0.395 \\
 & 720 &\textbf{ 0.344} &\textbf{ 0.345} & 0.358 &\underline{ 0.347} & 0.364 & 0.353 & 0.354 & 0.348 & 0.398 & 0.418 & 0.365 & 0.359 &\underline{ 0.345} & 0.381 & 0.377 & 0.427 & 0.403 & 0.428 & 0.414 & 0.410 & 0.419 & 0.428 \\
\multirow{-5}{*}{Weather} & avg &\textbf{ 0.243} &\textbf{ 0.273} &\underline{ 0.258} &\underline{ 0.278} & 0.272 & 0.291 & 0.259 & 0.281 & 0.259 & 0.315 & 0.259 & 0.287 & 0.265 & 0.317 & 0.292 & 0.363 & 0.309 & 0.360 & 0.288 & 0.314 & 0.338 & 0.382 \\ \midrule
\multicolumn{2}{c}{First Count} & \multicolumn{2}{c}{\textbf{43}} & \multicolumn{2}{c}{\underline{19}} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{4} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} \\ \bottomrule
\end{tabular}%
}
\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clccccccccccc} \toprule
\multicolumn{2}{c}{\textbf{Models}} & \textbf{Ours} & \textbf{\begin{tabular}[c]{@{}c@{}}Rlinear\\      XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PatchTST\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Crossformer \\      ICLR'XX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FEDformer \\      XXXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TimesNet\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DLinear \\      AAAI'xxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SCINet \\      xxxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FEDformer\\      XXXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Stationary\\      xxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Autoformer\\      XXXX\end{tabular}} \\ \midrule
 & SMAPE & \textbf{ 13.185} & 13.994 & \underline{ 13.258} & 13.392 & 13.728 & 13.387 & 16.965 & 13.717 & 13.728 & 13.717 & 13.974 \\
 & MASE & \textbf{ 2.955} & 3.015 & \underline{ 2.985} & 3.001 & 3.048 & 2.996 & 4.283 & 3.076 & 3.048 & 3.078 & 3.134 \\
\multirow{-3}{*}{Year} & OWA & \textbf{ 0.775} & 0.807 & \underline{ 0.781} & 0.787 & 0.803 & 0.786 & 1.058 & 0.807 & 0.803 & 0.807 & 0.822 \\ \midrule
 & SMAPE & \textbf{ 9.989} & 10.702 & 10.179 & 16.317 & 10.792 & \underline{ 10.1} & 12.145 & 10.845 & 10.792 & 10.958 & 11.338 \\
 & MASE & \underline{ 1.17} & 1.299 & \textbf{ 0.803} & 2.197 & 1.283 & 1.182 & 1.52 & 1.295 & 1.283 & 1.325 & 1.365 \\
\multirow{-3}{*}{Quarterly} & OWA & \underline{ 0.88} & 0.959 & \textbf{ 0.803} & 1.542 & 0.958 & 0.89 & 1.106 & 0.965 & 0.958 & 0.981 & 1.012 \\ \midrule
 & SMAPE & \textbf{ 12.453} & 13.363 & \underline{ 12.641} & 12.924 & 14.26 & 12.67 & 13.514 & 13.208 & 14.26 & 13.917 & 13.958 \\
 & MASE & \textbf{ 0.913} & 1.014 & \underline{ 0.93} & 0.966 & 1.102 & 0.933 & 1.037 & 0.999 & 1.102 & 1.097 & 1.103 \\
\multirow{-3}{*}{Monthly} & OWA & \textbf{ 0.861} & 0.94 & \underline{ 0.876} & 0.902 & 1.012 & 0.878 & 0.956 & 0.928 & 1.012 & 0.998 & 1.002 \\ \midrule
 & SMAPE & \textbf{ 4.565} & 5.437 & 4.946 & 5.439 & 4.954 & \underline{ 4.891} & 6.709 & 5.432 & 4.954 & 6.302 & 5.458 \\
 & MASE & \underline{ 3.144} & 3.706 & \textbf{ 2.985} & 3.69 & 3.264 & 3.302 & 4.953 & 3.583 & 3.264 & 4.064 & 3.865 \\
\multirow{-3}{*}{Others} & OWA & \textbf{ 0.976} & 1.157 & 1.044 & 1.16 & 1.036 & \underline{ 1.035} & 1.487 & 1.136 & 1.036 & 1.304 & 1.187 \\ \midrule
 & SMAPE & \textbf{ 11.636} & 12.473 & \underline{ 11.807} & 13.474 & 12.84 & 11.829 & 13.639 & 12.369 & 12.84 & 12.78 & 12.909 \\
 & MASE & \textbf{ 1.556} & 1.677 & 1.59 & 1.866 & 1.701 & \underline{ 1.585} & 2.095 & 1.677 & 1.701 & 1.756 & 1.771 \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Weighted\\      Average\end{tabular}} & OWA & \textbf{ 0.836} & 0.898 & \underline{ 0.851} & 0.985 & 0.918 & \underline{ 0.851} & \underline{ 0.851} & 0.894 & 0.918 & 0.93 & 0.939 \\ \midrule
\multicolumn{2}{c}{First Count} & \textbf{ 12} & 0 & \underline{ 3} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \bottomrule
\end{tabular}%
}
\end{table*}



% \begin{table*}[]
% \centering
% \caption{}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clccccccccccccccc}\toprule
% \multicolumn{2}{c}{\textbf{Models}} & \textbf{Ours} & \textbf{\begin{tabular}[c]{@{}c@{}}CARD \\      ICLR'24\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PatchTST\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Crossformer \\      ICLR'XX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FEDformer \\      XXXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RMLP \\      XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rlinear\\      XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MTS-mixer \\      XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LightTS \\      XXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DLinear \\      AAAI'xxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TimesNet\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SCINet \\      xxxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FEDformer\\      XXXXX\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Stationary\\      xxxx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Autoformer\\      XXXX\end{tabular}} \\ \midrule
%  & SMAPE & \textbf{ 13.185} & 13.302 & \underline{ 13.258} & 13.392 & 13.728 & 13.418 & 13.994 & 13.548 & 14.247 & 16.965 & 13.387 & 13.717 & 13.728 & 13.717 & 13.974 \\
%  & MASE & \textbf{ 2.955} & 3.016 & \underline{ 2.985} & 3.001 & 3.048 & 3.006 & 3.015 & 3.091 & 3.109 & 4.283 & 2.996 & 3.076 & 3.048 & 3.078 & 3.134 \\
% \multirow{-3}{*}{Year} & OWA & \textbf{ 0.775} & 0.786 & \underline{ 0.781} & 0.787 & 0.803 & 0.789 & 0.807 & 0.803 & 0.827 & 1.058 & 0.786 & 0.807 & 0.803 & 0.807 & 0.822 \\ \midrule
%  & SMAPE & \textbf{ 9.989} & \underline{ 10.031} & 10.179 & 16.317 & 10.792 & 10.382 & 10.702 & 10.128 & 11.364 & 12.145 & 10.1 & 10.845 & 10.792 & 10.958 & 11.338 \\ 
%  & MASE & \underline{ 1.17} & 1.176 & \textbf{ 0.803} & 2.197 & 1.283 & 1.234 & 1.299 & 1.196 & 1.328 & 1.52 & 1.182 & 1.295 & 1.283 & 1.325 & 1.365 \\
% \multirow{-3}{*}{Quarterly} & OWA & \underline{ 0.88} & 0.884 & \textbf{ 0.803} & 1.542 & 0.958 & 0.921 & 0.959 & 0.896 & 1 & 1.106 & 0.89 & 0.965 & 0.958 & 0.981 & 1.012 \\ \midrule
%  & SMAPE & \textbf{ 12.453} & 12.67 & \underline{ 12.641} & 12.924 & 14.26 & 12.998 & 13.363 & 12.717 & 14.014 & 13.514 & 12.67 & 13.208 & 14.26 & 13.917 & 13.958 \\ 
%  & MASE & \textbf{ 0.913} & 0.933 & \underline{ 0.93} & 0.966 & 1.102 & 0.976 & 1.014 & 0.931 & 1.053 & 1.037 & 0.933 & 0.999 & 1.102 & 1.097 & 1.103 \\
% \multirow{-3}{*}{Monthly} & OWA & \textbf{ 0.861} & 0.878 & \underline{ 0.876} & 0.902 & 1.012 & 0.909 & 0.94 & 0.879 & 0.981 & 0.956 & 0.878 & 0.928 & 1.012 & 0.998 & 1.002 \\ \midrule
%  & SMAPE & \textbf{ 4.565} & 5.33 & 4.946 & 5.439 & 4.954 & 5.098 & 5.437 & \underline{ 4.817} & 15.88 & 6.709 & 4.891 & 5.432 & 4.954 & 6.302 & 5.458 \\ 
%  & MASE & \underline{ 3.144} & 3.261 & \textbf{ 2.985} & 3.69 & 3.264 & 3.364 & 3.706 & 3.255 & 11.434 & 4.953 & 3.302 & 3.583 & 3.264 & 4.064 & 3.865 \\
% \multirow{-3}{*}{Others} & OWA & \textbf{ 0.976} & 1.075 & 1.044 & 1.16 & 1.036 & 1.067 & 1.157 & \underline{ 1.02} & 3.474 & 1.487 & 1.035 & 1.136 & 1.036 & 1.304 & 1.187 \\ \midrule
%  & SMAPE & \textbf{ 11.636} & 11.815 & \underline{ 11.807} & 13.474 & 12.84 & 12.473 & 12.473 & 11.892 & 13.252 & 13.639 & 11.829 & 12.369 & 12.84 & 12.78 & 12.909 \\
%  & MASE & \textbf{ 1.556} & 1.587 & 1.59 & 1.866 & 1.701 & 1.677 & 1.677 & 1.608 & 2.111 & 2.095 & \underline{ 1.585} & 1.677 & 1.701 & 1.756 & 1.771 \\ 
% \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Weighted\\      Average\end{tabular}} & OWA & \textbf{ 0.836} & \underline{ 0.85} & 0.851 & 0.985 & 0.918 & 0.898 & 0.898 & 0.859 & 1.051 & 0.851 & 0.851 & 0.894 & 0.918 & 0.93 & 0.939 \\  \midrule
% \multicolumn{2}{c}{First Count} & \textbf{ 12} & 0 & \underline{ 3} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}
